Radio Continuum Imaging of High Redshift Radio Galaxies

We present sensitive radio continuum images at high resolution of 37 radio galaxies at z > 2. The observations were made with the Very Large Array (VLA) at 4.7 GHz and 8.2 GHz, with typical resolutions of 0.45'' and 0.25'', respectively. Images of total and polarized intensity, and spectral index, are presented. Values for total and polarized intensity, and values of rotation measures, are tabulated for the hot spots in each source. The positions of the radio nuclei are tabulated, along with a variety of other source parameters. Analysis of the polarization data reveals large rotation measures (RMs) towards six sources. We argue that the RMs are due to magnetized, ionized gas local to the radio sources. The magnitude of the RMs are in excess of 1000 rad/m/m (rest frame) for these sources. Drawing an analogy to a class of lower redshift radio galaxies with extreme RMs, we speculate that these sources may be at the centers of dense, X-ray emitting cluster atmospheres.

==> SURVEYtab1.tex <==
%
%\raggedright
\pretolerance=10000  %no hyphenation
%%%%%%%%%% no number on first page, and pages at top of page.
\nopagenumbers
\headline {\ifnum\pageno=1 {} \else \hfill \folio \hfill\fi}
%
%
\def\doublespace {\smallskipamount=6pt plus0pt minus0pt
                  \medskipamount=12pt plus0pt minus0pt
                  \bigskipamount=24pt plus0pt minus0pt
                  \normalbaselineskip=24pt plus0pt minus0pt
                  \normallineskip=2pt
                  \normallineskiplimit=0pt
                  \jot=6pt
                  {\def\smallskip {\vskip\smallskipamount}}
                  {\def\medskip   {\vskip\medskipamount}}
                  {\def\bigskip   {\vskip\bigskipamount}}
                  {\setbox\strutbox=\hbox{\vrule 
                    height17.0pt depth7.0pt width 0pt}}
                  \parskip 12.0pt
                  \normalbaselines}
%
\magnification=\magstep1 
\hsize 6.8 truein
\vsize 9.3 truein
\hoffset -0.3 truein   
\voffset -0.3 truein
%\special{landscape}
%
%\doublespace
\parindent 0.0pt
% TABLE
\vbox{
\centerline {\bf Table 1:  Source Parameters}
\bigskip
\hrule
\vskip3truept
\hrule
\tabskip=1em plus 2em minus.5em
\newdimen\digitwidth
\setbox0=\hbox{\rm0}
\digitwidth=\wd0
\catcode`?=\active
\def?{\kern\digitwidth}
\halign to
\hsize{\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil#  \cr
\noalign{\vskip 1 truemm}
Source~~  &  z~~ &  Cat$^a$ & R$^b$ &  Size$^c$ 
&  F$_{1.5}^d$ & F$_{4.7}^e$ & F$_{8.2}^f$ & Ref$^g$ \cr
\noalign{\vskip 3 truemm}
B1950~~ & ~ & ~ & mag & arcsec & mJy & mJy & mJy &  ~ \cr
\noalign{\vskip 1 truemm \hrule \vskip 1 truemm}
0015$-$229 & 2.010 & ML & 23.1 & 13.9 & 343 & 72 & 25  & 10 \cr
0030$-$219 & 2.168 & ML & 23.8  &  $<$0.3 & 251 & 87 & 48 & 3,10 \cr
0140$-$257 & 2.640 & ML & 23.3  & 4.2 & 203 & 47 & 23 &  7,10 \cr
0156$-$252 & 2.090 & ML & 22.9  & 8.3 & 343 & 112 & 60 &  3,10 \cr
0200+015 & 2.229 & TX & 22.1 &   5.6 & 183 & 50 & 21 & 2 \cr
0211$-$122 & 2.336 & TX & 22.7   & 17.0 & 189 & 54 & 24  &  2 \cr
0214+183 & 2.130 & TX & 21.5 & 7.5 & 300 & 85 & 42 &  2 \cr
0316$-$257 & 3.130 & ML & 22.6  & 7.6 & 308 & 101 & 49  & 3,10 \cr
0406$-$244 & 2.440 & ML & 22.7   & 10.0 & 374 & 108 & 51  & 7,10 \cr
0417$-$181 & 2.773 & TX & 21.7  & 4.3 & 273 & 72 & 36 &  2 \cr
0448+091 & 2.037 & TX & 23.1   & 24.0 & 129 & 29 & 7 &  2 \cr
0508+606 & 3.791 & 4C & 23.2   & 9.0 & 146 & 26 & 11 &  9 \cr
0731+438 & 2.429 & B3 & 23.0  & 10.8 & 690 & 170 & 65 & 6 \cr
0744+464 & 2.926 & B3 & 22.5 & 1.9 & 503 & 152 & 78  &  6 \cr
0748+134 & 2.419 & TX & 22.5  & 14.6 & 134 & 31 & 8  &  2 \cr
0828+193 & 2.572 & TX & 20.7   &  12.8 & 72 & 22 & 9  & 2 \cr
0943$-$242 & 2.923 & TX & 22.3  & 3.9 & 245 & 55 & 21  & 2 \cr
1106$-$258 & 2.430 & ML & 21.2 & 5.0 & 210 & 46 & 21  & 10 \cr
1113$-$178 & 2.239 & TX & 21.4 & 12.0 & 256 & 76 & 39  & 2  \cr
1138$-$262 & 2.156 & PK & 21.4 &  15.8 & 600 & 153 & 55 &  2 \cr
1232+397 & 3.221 & 6C & 22.4   & 8.0 & 250 & 43 & 16 &  8 \cr
1324$-$262 & 2.280 & ML & 23.3 & 1.8 & 520 & 98 & 48 & 10 \cr
1345+245 & 2.889 & 4C & 22.7   & 2.3 & 506 & 115 & 54  &  9 \cr
1410$-$001 & 2.363 & 4C & 22.6    & 24.0 & 179 & 57 & 27 &  4 \cr
1435+633 & 4.252 & 8C & 24.1 &  4.3 & 450 & 70 & 25  &  1 \cr
1436+157 & 2.550 & TX & 19.6 &  5.5 & 138 & 47 & 25 &  2 \cr
1545$-$234 & 2.755 & TX & 22.7   & 7.5 & 222 & 59 & 21 &  2 \cr
1744+183 & 2.281 & MG & 23.0 & 7.5 & 1100 & 333 & 174 & 11 \cr
1809+407 & 2.267 & 4C & 21.2 &  4.0 & 469 &  75 & 27 & 9 \cr
1931+480 & 2.348 & 4C & 22.1 &  14.0 & 334 & 90 & 43 & 9 \cr
2025$-$218 & 2.630 & ML & 22.1   & 5.1 & 325 & 95 & 51 & 3,10 \cr 
2036$-$254 & 2.000 & ML & 23.5 & 7.6 & 350 & 94 & 48 & 10 \cr
2105+236 & 2.479 & 4C & 23.2 &  53.0 & 343 & 62 & 28  &  9 \cr
2139$-$292 & 2.550 & ML & 21.2 & 8.0 & 440  & 117 & 59 & 10 \cr
2141+192 & 3.594 & MG & 23.3 &  8.9 & 146 & 67 & 28 &   1 \cr
2202+128 & 2.704 & TX & 23.1 &  4.2 & 161 & 52 & 22 &  2 \cr
2251$-$089 & 1.986 & PK & 22.8 & 3.0 & 388 & 110 & 63 & 2 \cr
\noalign{\medskip}
\noalign{\hrule}
}
}
\parskip 0.0in
\parindent 0pt

~$^a$Catalogs: ML = Molonglo (Large etal. 1981); 
PK = Parkes (Bolton etal 1979), TX = Texas
(Douglas etal 1980); Cambridge: 4C, 6C, 8C (Baldwin etal 1985, 
Hales etal 1995, Rees 1990); 
MG = MIT-Greenbank (Gregory and Condon 1991, Becker etal 1991); 
B3 = Third Bologna (Vigotti etal 1989).

~$^b$R = optical R band magnitude

~$^c$Maximum source size in arcseconds 

~$^d$F$_{1.5}$ = flux density at 1.5 GHz

~$^e$F$_{4.7}$ = flux density at 4.7 GHz

~$^f$F$_{8.2}$ = flux density at 8.2 GHz

~$^g$References: 1. Lacy {\sl etal.} 1994,
2. Rottgering 1993, 3. McCarthy {\sl et al.} 1990, 
4. Rottgering {\sl etal.}  1996, 6. McCarthy 1991,
7. McCarthy {\sl etal.} 1991, 8. Eales {\sl et al.} 1993,
9. Chambers {\sl et al.} 1996, 10. McCarthy {\sl et al.} 1996,
11. Eales and Rawlings 1993.

\vfill\eject
\bye



==> SURVEYtab2.tex <==
%
%\raggedright
\pretolerance=10000  %no hyphenation
%%%%%%%%%% no number on first page, and pages at top of page.
\nopagenumbers
\headline {\ifnum\pageno=1 {} \else \hfill \folio \hfill\fi}
%
%
\def\doublespace {\smallskipamount=6pt plus0pt minus0pt
                  \medskipamount=12pt plus0pt minus0pt
                  \bigskipamount=24pt plus0pt minus0pt
                  \normalbaselineskip=24pt plus0pt minus0pt
                  \normallineskip=2pt
                  \normallineskiplimit=0pt
                  \jot=6pt
                  {\def\smallskip {\vskip\smallskipamount}}
                  {\def\medskip   {\vskip\medskipamount}}
                  {\def\bigskip   {\vskip\bigskipamount}}
                  {\setbox\strutbox=\hbox{\vrule 
                    height17.0pt depth7.0pt width 0pt}}
                  \parskip 12.0pt
                  \normalbaselines}
%
\magnification=\magstep0
\hsize 6.7 truein
\vsize 9.6 truein
\hoffset -0.3 truein   
\voffset -0.4 truein
%\special{landscape}
%
%\doublespace
\parindent 0.0pt
% TABLE
\vbox{
\centerline {\bf Table 2:  Core Parameters and Restoring Beams}
\bigskip
\hrule
\vskip3truept
\hrule
\tabskip=1em plus 2em minus.5em
\newdimen\digitwidth
\setbox0=\hbox{\rm0}
\digitwidth=\wd0
\catcode`?=\active
\def?{\kern\digitwidth}
\halign to
\hsize{\hfil#&\hfil#&\hfil#&\hfil#&\hfil# \cr
\noalign{\vskip 1 truemm}
Source & Core Position~~~~~~~~~~ & F$_{8.2}^a$~~ & $\alpha_{4.7}^{8.2}$ & CF$_{20}^b$  \cr
\noalign{\vskip 3 truemm}
~ & B = B1950,~~ J = J2000~~~~ & mJy/beam & ~ & $\%$ \cr
\noalign{\vskip 1 truemm \hrule \vskip 1 truemm}
0015$-$229 & B00$^h$ 15$^m$ 26.43$^s$~~~$-$22$^o$ 54$'$ 43.3$''$ & U1.59 & $-$1.3 & 5.6  \cr
0030$-$219 & B00$^h$ 30$^m$ 53.87$^s$~~~$-$21$^o$ 58$'$ 34.3$''$ & U44.90 & $-$1.0 & 100.0 \cr
0140$-$257 & B01$^h$ 40$^m$ 21.18$^s$~~~$-$25$^o$ 45$'$ 39.8$''$ & 0.52 & $-$0.4 & 1.6  \cr
0156$-$252 & B01$^h$ 56$^m$ 15.06$^s$~~~$-$25$^o$ 14$'$ 05.9$''$ & 6.58 & $-$0.7 & 10.0  \cr
0200+015 & $-$ & $-$ & $-$ & $-$  \cr
0211$-$122 & J02$^h$ 14$^m$ 17.37$^s$~~~$-$11$^o$ 58$'$ 46.8$''$ & U1.23 & $-$1.0 & 3.8 \cr
0214+183 & J02$^h$ 17$^m$ 25.80$^s$~~~+18$^o$ 37$'$ 02.9$''$ & 0.74 & $-$0.2 & 1.4  \cr
0316$-$257 & $-$ & $-$ & $-$ & $-$  \cr
0406$-$244 & B04$^h$ 06$^m$ 44.44$^s$~~~$-$24$^o$ 26$'$ 07.9$''$ & 1.59 & $-$0.8 & 2.6  \cr
0417$-$181 & J04$^h$ 19$^m$ 43.68$^s$~~~$-$18$^o$ 01$'$ 52.5$''$ & X0.26 & $-$0.7 & 0.6  \cr
0448+091 & $-$ & $-$ & $-$ & $-$  \cr
0508+606 & B05$^h$ 08$^m$ 26.14$^s$~~~+60$^o$ 27$'$ 17.1$''$ & U0.21 & $-$1.7 & 2.1  \cr
0731+438 & B07$^h$ 31$^m$ 49.35$^s$~~~+43$^o$ 50$'$ 59.1$''$ & U0.64 & $-$1.5 & 0.9  \cr
0744+464 & B07$^h$ 44$^m$ 07.08$^s$~~~+46$^o$ 26$'$ 24.6$''$ & X1.37 & $-$0.4 & 1.2  \cr
0748+134 & $-$ & $-$ & $-$ & $-$  \cr
0828+193 & B08$^h$ 28$^m$ 01.08$^s$~~~+19$^o$ 23$'$ 23.7$''$ & 2.81 & $-$0.7 & 21.0 \cr
0943$-$242 & $-$ & $-$ & $-$ & $-$  \cr
1106$-$258 & B11$^h$ 06$^m$ 03.99$^s$~~~$-$25$^o$ 48$'$ 49.9$''$ & U0.21 & $-$1.5 & 9.9 \cr
1113$-$178 & J11$^h$ 16$^m$ 14.67$^s$~~~$-$18$^o$ 06$'$ 22.8$''$ & 3.63 & $-$0.7 & 7.9  \cr
1138-262 & J11$^h$ 38$^m$ 17.54$^s$~~~$-$26$^o$ 12$'$ 30.44$''$ & U1.98 & $-$1.3 & 3.1 \cr
1232+397 & B12$^h$ 32$^m$ 39.14$^s$~~~+39$^o$ 42$'$ 08.8$''$ & 0.35 & $-$0.2 & 0.7  \cr
1324$-$262 & B13$^h$ 24$^m$ 08.79$^s$~~~$-$26$^o$ 16$'$ 08.8$''$ & X0.86 & $-$0.3 & 1.4 \cr
1345+245 & B13$^h$ 45$^m$ 54.75$^s$~~~+24$^o$ 30$'$ 45.2$''$ & X0.51 & $-$0.6 & 0.7 \cr
1410$-$001 & J14$^h$ 13$^m$ 15.13$^s$~~~$-$00$^o$ 22$'$ 59.5$''$ & 2.27 & $-$0.7 & 6.7  \cr
1435+633 & J14$^h$ 36$^m$ 37.22$^s$~~~+63$^o$ 19$'$ 14.0$''$ & U1.31 & $-$1.3  & 3.3  \cr
1436+157 & B14$^h$ 36$^m$ 43.03$^s$~~~+15$^o$ 44$'$ 12.7$''$ & 0.69 & $-$0.6 & 2.1  \cr
1545$-$234 & J15$^h$ 48$^m$ 17.47$^s$~~~$-$23$^o$ 37$'$ 00.9$''$ & U3.31 & $-$1.1 & 11.0  \cr
1744+183 & $-$ & $-$ & $-$ & $-$  \cr
1809+407 & $-$ & $-$ & $-$ & $-$  \cr
1931+480 & B19$^h$ 31$^m$ 40.45$^s$~~~+48$^o$ 05$'$ 12.4$''$ & 0.40 & $-$0.4 & 0.6  \cr
2025$-$218 & B20$^h$ 25$^m$ 04.26$^s$~~~$-$21$^o$ 50$'$ 55.2$''$ & X0.38 & $-$0.9 & 0.7  \cr
2036$-$254 & B20$^h$ 36$^m$ 26.27$^s$~~~$-$25$^o$ 25$'$ 7.68$''$ & UX0.31 & 0.2 & 0.5 \cr
2105+236 & B21$^h$ 05$^m$ 00.97$^s$~~~+23$^o$ 19$'$ 37.8$''$ & 4.95 & $-$0.9 & 14.6  \cr
2139$-$292 & $-$ & $-$ & $-$ & $-$  \cr
2141+192 & $-$ & $-$ & $-$ & $-$  \cr
2202+128 & B22$^h$ 02$^m$ 47.87$^s$~~~+12$^o$ 50$'$ 56.3$''$ & U0.14 & $-$2.5 & 0.9  \cr
2251$-$089 & J22$^h$ 53$^m$ 40.38$^s$~~~$-$08$^o$ 40$'$ 43.0$''$ & 22.20 & $-$0.8 & 33.0  \cr
\noalign{\medskip}
\noalign{\hrule}
}
}
\parskip 0.0in

~$^a$Surface brightness in mJy/beam at 8.2 GHz, as measured on the 
images convolved to the resolution of the corresponding 
4.7 GHz image, unless preceeded by
an `X', implying that the source was small, and 
the measurement was made using the full resolution 8.2GHz  image.
A `U' means that the core identification is uncertain,
either due to confusion, low S/N, or spectral index $\le$ $-$1.0.

~$^b$Core Fraction = ratio of core flux density to total source flux 
density at a rest frame frequency of 20 GHz, in percentage.

\vfill\eject
\bye



==> SURVEYtab3.tex <==
%\raggedright
\nopagenumbers
\pretolerance=10000  %no hyphenation
%%%%%%%%%% no number on first page, and pages at top of page.
\nopagenumbers
\headline {\ifnum\pageno=1 {} \else \hfill \folio \hfill\fi}
%
%
\def\doublespace {\smallskipamount=6pt plus0pt minus0pt
                  \medskipamount=12pt plus0pt minus0pt
                  \bigskipamount=24pt plus0pt minus0pt
                  \normalbaselineskip=24pt plus0pt minus0pt
                  \normallineskip=2pt
                  \normallineskiplimit=0pt
                  \jot=6pt
                  {\def\smallskip {\vskip\smallskipamount}}
                  {\def\medskip   {\vskip\medskipamount}}
                  {\def\bigskip   {\vskip\bigskipamount}}
                  {\setbox\strutbox=\hbox{\vrule 
                    height17.0pt depth7.0pt width 0pt}}
                  \parskip 12.0pt
                  \normalbaselines}
%
\magnification=\magstep0
\hsize 9.1 truein
\vsize 5.5 truein
\hoffset 0 truein   
\voffset 0 truein
\special{landscape}
%
%\doublespace
\parindent 0.0pt
% TABLE
\vbox{
\centerline {\bf Table 3: Hot Spots  Parameters$^a$}
\hrule
\vskip3truept
\hrule
\tabskip=1em plus 2em minus.5em
\newdimen\digitwidth
\setbox0=\hbox{\rm0}
\digitwidth=\wd0
\catcode`?=\active
\def?{\kern\digitwidth}
\halign to
\hsize{\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil#&\hfil# \cr
\noalign{\vskip 3 truemm}
\noalign{\hskip 4.2 truecm Southern Hot Spot \hskip 7.0truecm Northern Hot Spot \hfil}
\noalign{\vskip 1 truemm \hrule \vskip 1 truemm}
Source  &  I$_{4.7}^b$ & $\alpha_{4.7}^{8.2c}$  & FP$_{4.7}^d$ &  FP$_{8.2}^e$ & RM$^f$ & 
I$_{4.7}$ & $\alpha_{4.7}^{8.2}$  & FP$_{4.7}$ &  FP$_{8.2}$ & RM \cr
\noalign{\vskip 3 truemm}
~ & mJy/beam & ~ & $\%$ & $\%$ & rad m$^{-2}$ &  mJy/beam & ~ & $\%$ & $\%$ & rad m$^{-2}$ \cr
\noalign{\vskip 1 truemm \hrule \vskip 1 truemm}
0015$-$229 &  3.56 & $-$1.7 & 12.4 & 10.0 &  59 & 18.10 & $-$1.3 & 3.3 & 3.0 &  90 \cr
0030$-$219 &  41.57 & $-$1.0 & $-$  & $-$  & $-$  &   $-$ &   $-$ &   $-$ &   $-$ & $-$  \cr
0140$-$257 &  24.75 & $-$1.3 & 5.4 & 4.8 & 1  & 8.21 & $-$1.4 & 7.9 & 7.3 &  87   \cr
0156$-$252 &  3.29 & $-$1.4 & $-$   & $-$  & $-$ &  60.47 & $-$1.1 & 4.6 & 4.5 &  77  \cr
0200+015 &  21.41 & $-$1.7 & 17.9 & 14.8 &  $-$32 & 13.00 & $-$1.4 & 6.7 & 5.3 &  32  \cr
0211$-$122 &  19.14 & $-$1.2 & 12.9 & 11.3 & 14 &  6.73 & $-$1.4 &  $-$ &  $-$ &  $-$  \cr
0214+183 &   4.92 & $-$1.4 & $-$  & $-$  & $-$  & 58.44 & $-$1.2  & 8.5 & 15.0 &  39  \cr
0316$-$257 &  54.61 & $-$1.4 & 1.0 &  0.9 &  32 & 30.54 & $-$1.4 & 1.6 & 5.0 &  45  \cr
0406$-$244 &  17.89 & $-$1.7 & 1.7 & 4.6 & 403 & 55.56 & $-$1.3 & 6.9 & 6.0 &  57  \cr
0417$-$181 &  46.45 & $-$1.2 & 1.1 & 1.5 &  $-$ & 17.34 & $-$1.6 & $-$  & $-$  &  $-$  \cr
0448+019 &   3.66 & $-$1.7 &  $-$ &  $-$ &  $-$  &  1.55 & $-$1.9  & $-$ &  $-$ &  $-$  \cr
0508+606 &   1.88 & $-$2.8 & $-$ &  $-$ &   $-$ & 12.82 & $-$1.4 &  9.0 & 8.1 &  $-$62  \cr
0731+438 &  64.22 & $-$1.2 & 6.0 & 5.2 &  32 & 16.70 & $-$1.5 & 1.0 &  $-$ &   $-$  \cr
0744+464 &  17.66 & $-$1.5 & $-$ &  $-$ &   $-$ & 121.86 & $-$1.2 & 0.9 & 6.0 & $-$280  \cr
0748+134 &   3.17 & $-$1.3 & $-$  & $-$ &   $-$ &  3.00 & $-$1.9 &  $-$ &  $-$ &  $-$  \cr
0828+193 &   6.35 & $-$2.0 & 6.6 & $-$  &  $-$ &  2.45 & $-$1.9 & 29.0 &  $-$  &  $-$  \cr
0943$-$242 &   8.93 & $-$1.6 & 2.9 & $-$ &   $-$ & 40.26 & $-$1.7 & $-$  & 3.9 &  $-$  \cr
1106$-$258 &  11.61 & $-$1.5 & 17.4 & 14.0 &  30 & 29.42 & $-$1.5 & 2.7 & 4.3 &  30 \cr
1113$-$178 &  14.75 & $-$1.3 & 5.2 & 2.0 &  17 & 20.66 & $-$1.1 & 15.5  & 15.0 &  47  \cr
1138$-$262 &  21.10 & $-$1.7 & 2.9 & 8.7 &  63 & 32.23 & $-$1.9 & 4.4 & 6.8 & $-$624  \cr
1232+397 &   9.56 & $-$1.5 & 11.6 & 14.5 &  59 & 12.74 & $-$1.5 & 14.3  & 11.3 & $-$63  \cr
1324$-$262 &  54.61 & $-$1.2 & 8.1 & 8.6 &  169 &  29.86 & $-$1.6 &  $-$ & 1.5 &  $-$ \cr
1345+245 &  27.16 & $-$1.7 & $-$ &  2.0 &  $-$ & 71.41 & $-$1.3 & 5.1 & 6.1 &  47  \cr
1410$-$001 &   9.09 & $-$1.4 & 6.1  & 3.5  & 30 & 16.25 & $-$1.2 & 9.9 & 9.1 &   0  \cr
1435+633 &  48.39 & $-$2.0 & $-$  & 1.3 &  $-$ & 15.53 & $-$1.9 &  $-$ &  $-$  &  $-$  \cr
1436+157 &  22.67 & $-$0.9 & 10.3 & 13.6 & 111 &  5.18 & $-$1.3 &  $-$ & 7.3 &  $-$  \cr
1545$-$234 &  15.22 & $-$1.7 & $-$ &  $-$ &   $-$ & 16.20 & $-$2.0 &  $-$  & $-$ &   $-$  \cr
1744+183 & 161.48 & $-$1.1 & 5.9 & 11.0 &  76 & 90.91 & $-$1.0 & 18.0 & 23.0 &  64 \cr
1809+407 &  18.07 & $-$1.5 & 5.0 & 3.9 & 118 & 38.14 & $-$1.7 &  $-$ &  $-$ &  $-$  \cr
1931+480 &  43.57 & $-$1.2 & 6.9 & 12.6 & $-$28 &  1.65 & $-$1.8 &  $-$ &  $-$  & $-$   \cr
2025$-$218 &  24.52 & $-$1.1 & 8.6 & 7.9 &   9 & 23.42 & $-$1.3 & 2.3  & 5.7  & 69   \cr
2036$-$254 &  26.92 & $-$1.6 & 3.5 & 2.9 & $-$389 & 48.82 & $-$1.0 & 19.0 & 17.1 &  $-$6 \cr
2105+236 &  15.57 & $-$1.1 & 10.5 &  8.0 & $-$190 &  5.79 & $-$1.7 &  6.4 &  $-$ &  $-$  \cr
2139$-$292 &  40.20 & $-$1.6 & 4.0 & 3.4 & $-$56 & 43.62 & $-$1.3 & 15.0 & 10.4 &  $-$5 \cr
2141+192 &  21.98 & $-$1.6 & $-$ &  $-$ &   $-$ & 34.99 & $-$1.6 &  $-$ &  $-$ &   $-$  \cr
2202+128 &  19.00 & $-$1.2 & 9.4 & 5.5 & $-$12 & 12.16 & $-$1.5 & 5.6 & 3.5 & $-$188  \cr
2251$-$089 &  46.37 & $-$1.0 & $-$  & $-$  & $-$ &   8.17 & $-$0.8 & 7.3 & 5.1 &  $-$4  \cr
\noalign{\medskip}
\noalign{\hrule}
}
}
\parskip 0.0in
\parindent 0pt

\vfill\eject

~$^a$Columns  2 to 6 correspond to the southern hot spot in each source. Columns
7 to 11 correspond to the northern hot spot in each source. All values at 8.2 GHz
were measured on images convolved to the resolution of the corresponding
4.7 GHz image. A blank entry means a non-detection at 4$\sigma$.

~$^b$I$_{4.7}$ = peak surface brightness in mJy/Beam at 4.7 GHz 

~$^c$$\alpha_{4.7}^{8.2}$ = spectral index between 4.7 GHz and 8.2 GHz

~$^d$FP$_{4.7}$ = fractional polarization at 4.7 GHz

~$^e$FP$_{8.2}$ = fractional polarization at 8.2 GHz

~$^f$RM = rotation measure in rad m$^{-2}$, calculated
using observed frequencies without correction for redshift.
RM magnitudes $<$ 100 rad m$^{-2}$ are unreliable, as discussed in the text.


\vfill\eject
\bye


